N\'eron models of formally finite type

We introduce N\'eron models of formally finite type for uniformly rigid spaces, and we prove that they generalize the notion of formal N\'eron models for rigid-analytic groups as it was defined by Bosch and Schl\"oter. Using this compatibility result, we give examples of uniformly rigid groups whose N\'eron models are not of topologically finite type.

==> preamble.tex <==
\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{dsfont}
\usepackage{stmaryrd}
\usepackage{exscale}
\usepackage{extraipa}
\usepackage{tocloft}
\usepackage[dvips]{graphicx}
\usepackage{makeidx}
%\usepackage{multind}
%\usepackage{drftcite}

\usepackage[latin9]{inputenc}
\usepackage{ae}
%\usepackage{t1enc}
%\usepackage[german]{babel}

\usepackage{a4}
\usepackage{fancyhdr}
\usepackage[compact,nobottomtitles,rigidchapters]{titlesec}

\usepackage{theorem}
\usepackage{diagrams}

%\usepackage[bottom]{footmisc}

\setlength{\cftparskip}{0pt} 

%\makeindex{symbols}
\makeindex%{main}



\ifthenelse{\boolean{hyper}}
    {\usepackage[pdftex]{hyperref}}
    {}


\ifthenelse{\boolean{smallbook}}
   {\setboolean{PSdiagram}{true}}
   {}

\ifthenelse{\boolean{PSdiagram}}
  {\setboolean{debug}{false}}
  {}



\ifthenelse{\boolean{debug}}
   { \usepackage{srcltx}
%     \usepackage{showkeys}
   }
   {}


% set depths for numbering and toc

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}

\titleformat{\part}[block]{\Huge\bf}{\thepart. }{0pt}{}

\titleformat{\chapter}[block]{\LARGE\bf}{\thechapter. }{0.5em}{}

\titlespacing*{\chapter}{0in}{-2ex}{2in}
\titlespacing*{\section}{0in}{*4}{*2}
\titlespacing*{\subsection}{0in}{*4}{*2}





\let\oldsection\section
\let\oldsubsection\subsection


\newcommand\mysection[1]{\renewcommand{\bottomtitlespace}{0.42\textheight}\oldsection{#1}}
\newcommand\mysubsection[1]{\renewcommand{\bottomtitlespace}{0.33\textheight}\oldsubsection{#1}}

\let\section\mysection
\let\subsection\mysubsection


%Kopf- und Fußzeilen


\pagestyle{fancy}

\fancyhead{} %
\fancyfoot{} %
\fancyhead[LE]{\thepage   \hspace{0.5in} \leftmark} %
\fancyhead[RO]{\rightmark \hspace{0.33in} \thepage} %


%\renewcommand{\chaptermark}[1]{\markboth{#1}{}}
\renewcommand{\sectionmark}[1]{\markright{\thesection.\ #1}}
\renewcommand{\headrulewidth}{0.5pt}
\renewcommand{\headheight}{16pt}



\fancypagestyle{plain}{
  \fancyhf{}
}


\setlength{\headsep}{16pt} %


\ifthenelse{\boolean{smallbook}}
  {
   % Ränder für Buch
   % Aufruf dvips -x 850 -Ppdf alggeo
   %        dvipdfm -p a4 -m 0.85 alggeo
   \setlength{\topmargin}{0cm}
   \setlength{\oddsidemargin}{-0.5cm} %
   \setlength{\evensidemargin}{3.8cm} %   für a4
   %\setlength{\evensidemargin}{2.5cm} %  für a4wide
  }
  {}


\renewcommand\textrm[1]{{\rm #1}}

\setlength{\parskip}{\medskipamount}
\setlength\parindent{0.0cm}

\newlength{\listindent}
\setlength{\listindent}{\parindent}

\newcommand\romanenum{\renewcommand{\labelenumi}{\textup{(}\roman{enumi}\textup{)}}}
\newcommand\alphenum{\renewcommand{\labelenumi}{\textup{(}\alph{enumi}\textup{)}}}


\newcommand\enumroman[1]{{\rm(\/\textit{\roman{#1}}\/)}}
\newcommand\enumarabic[1]{\arabic{#1}.}
\newcounter{enumcounter}
\newcommand\enum[1]{\setcounter{enumcounter}{#1}\enumroman{enumcounter}}
\newcommand\impl[2]{\enum{#1} $\then$ \enum{#2}}
\newcommand\Impl[2]{\par\noindent\enum{#1} $\then$ \enum{#2}}



\newenvironment{items}
   {\begin{list}{\textbullet} {
                    \setlength{\topsep}{0.1ex plus0.1ex minus0.1ex}
                    \setlength{\itemsep}{0.1ex plus0.1ex minus0.1ex}
                    \setlength{\parsep}{0.1ex plus0.1ex minus0.1ex}
                    \setlength{\itemindent}{0in}
                    \setlength{\labelwidth}{1ex}
                    \setlength{\leftmargin}{\listindent}
                    \setlength{\partopsep}{\medskipamount} } }
   {\end{list}}



\newenvironment{enumprop}
   {\begin{list}{\enumroman{enumiv}}{\usecounter{enumiv}
                      \setlength{\topsep}{0.8ex plus0.1ex minus0.1ex}
                      \setlength{\itemsep}{0.1ex plus0.1ex minus0.1ex}
                      \setlength{\parsep}{0.1ex plus0.1ex minus0.1ex}
                      \setlength{\itemindent}{0in}
                      \setlength{\labelwidth}{2.5em}
                      \setlength{\leftmargin}{2\listindent}
                      \setlength{\partopsep}{\medskipamount} } }
   {\end{list}}

\newenvironment{enumsrm}
   {\begin{list}{\enumroman{enumiv}}{\usecounter{enumiv}
                      \setlength{\topsep}{0.1ex plus0.1ex minus0.1ex}
                      \setlength{\itemsep}{0.1ex plus0.1ex minus0.1ex}
                      \setlength{\parsep}{0.1ex plus0.1ex minus0.1ex}
                      \setlength{\itemindent}{0in}
                      \setlength{\labelwidth}{2.5em}
                      \setlength{\leftmargin}{2\listindent}
                      \setlength{\partopsep}{\medskipamount} } }
   {\end{list}}



\newenvironment{enumsarabic}
   {\begin{list}{\enumarabic{enumiv}}{\usecounter{enumiv}
                      \setlength{\topsep}{0.1ex plus0.1ex minus0.1ex}
                      \setlength{\itemsep}{0.1ex plus0.1ex minus0.1ex}
                      \setlength{\parsep}{0.1ex plus0.1ex minus0.1ex}
                      \setlength{\itemindent}{0in}
                      \setlength{\labelwidth}{3ex}
                      \setlength{\leftmargin}{\listindent}
                      \setlength{\partopsep}{\medskipamount} } }
   {\end{list}}

\newenvironment{univprop}
   {\begin{list}{}  {\setlength{\topsep}{\medskipamount}
                    \setlength{\itemsep}{0ex}
                    \setlength{\parsep}{0.5ex plus0.2ex minus0.2ex}
                    \setlength{\itemindent}{0in}
                    \setlength{\listparindent}{0in}
                    \setlength{\labelwidth}{0ex}
                    \setlength{\leftmargin}{1.5\listindent}
                    \setlength{\rightmargin}{1.5\listindent}
                    \setlength{\partopsep}{\medskipamount} }
      \item}
   {\end{list}}


\newenvironment{mathprop}
   {\begin{list}{}  {\setlength{\topsep}{\medskipamount}
                    \setlength{\itemsep}{0ex}
                    \setlength{\parsep}{0.5ex plus0.2ex minus0.2ex}
                    \setlength{\itemindent}{0in}
                    \setlength{\listparindent}{0in}
                    \setlength{\labelwidth}{0ex}
                    \setlength{\leftmargin}{1.5\listindent}
                    \setlength{\rightmargin}{1.5\listindent}
                    \setlength{\partopsep}{\medskipamount} }
      \item\it}
   {\end{list}}


%Optionen für Diagramme

\ifthenelse{\boolean{PSdiagram}} %
 {
  \diagramstyle[height=0.3in,width=0.4in,labelstyle=\scriptstyle,dpi=1200,nohug,PostScript=dvips]
 }{
  \diagramstyle[height=0.3in,width=0.4in,labelstyle=\scriptstyle,dpi=600,nohug,noPostScript]
 }

\newcommand\varhspace[1][1em]{\hspace{0em plus#1 minus0.3em}}
\newcommand\negproof{\vspace{-8ex}\par}

\newcommand\Proofpart[1]{\par\noindent\textit{#1}}
\newcommand\proofpart[1]{\textit{#1}}
\newcommand\statement[1]{\proofpart{Aussage \enum{#1}}}
\newcommand\Statement[1]{\Proofpart{Aussage \enum{#1}}}


\hyphenation{noe-thersch noe-ther-sche noe-ther-schen Ver-bin-dungs-mor-phis-mus Ver-bin-dungs-mor-phis-men}


%Allgemeine Definitionen

\newarrowtail{<=}\Leftarrow\Rightarrow\Uparrow\Downarrow

\newarrow{Corresponds} <--->
\newarrow{Equal} =====
\newarrow{Equiv} {<=}==={=>}
\newarrow{Dash} {}{dash}{}{dash}{}
\newarrow{Dashinto} C{dash}{}{dash}>
\newarrow{Dashonto} {}{dash}{}{dash}{>>}
\newarrow{Dotmapsto} {mapsto}...>



\newarrow{CTo} ----{->}
\newarrow{CMapsto} |---{->}
\newarrow{CInto} C---{->}
\newarrow{COnto} ----{->>}

\def\NWpok{\NWpbk}



\newcommand\diagramiso{\hbox{\lower1.5ex\hbox{$_\sim$}}}



\theoremstyle{change} %
\theorembodyfont{\it}
	

\newtheorem{defi}{Definition.}[subsection]
\newtheorem{defi*}{Definition.}
\newtheorem{defnprop}[defi]{Definition und Satz.}
\newtheorem{lem}[defi]{Lemma.}
\newtheorem{prop}[defi]{Proposition.}
\newtheorem{theorem}[defi]{Theorem.}
\newtheorem{cor}[defi]{Corollary.}
\newtheorem{remark}[defi]{Remark.}
\newtheorem{remarkdefi}[defi]{Remark and Definition.}
\newtheorem{observation}[defi]{Observation.}
\newtheorem{convention}[defi]{Convention.}
\newtheorem{notation}[defi]{Notation.}
\newtheorem{examples}[defi]{Examples.}
\newtheorem{example}[defi]{Example.}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
                                 
\newenvironment{interlude}{\begin{trivlist}\setlength\topsep{\theorempreskipamount}\item}{\end{trivlist}}
\newenvironment{smallinterlude}{\begin{trivlist}\setlength\topsep{\theorempreskipamount}\item\small}{\normalsize\end{trivlist}}

%\newenvironment{remark}{\begin{interlude}\pagebreak[2]\noindent\textit{Remark.\ }\nopagebreak}{\end{interlude}}
%\newenvironment{observation}{\begin{interlude}\pagebreak[2]\noindent\textit{Observation.\ }\nopagebreak}{\end{interlude}}
%\newenvironment{convention}{\begin{interlude}\pagebreak[2]\noindent\textit{Convention.\ }\nopagebreak}{\end{interlude}}
\newenvironment{remarks}{\begin{interlude}\pagebreak[2]\noindent\textbf{Bemerkungen.\ }\nopagebreak\begin{enumsrm}\nopagebreak}{\end{enumsrm}\end{interlude}}
\newenvironment{remarks*}{\begin{interlude}\pagebreak[2]\noindent\textbf{Bemerkungen.\ }\nopagebreak}{\end{interlude}}

%\newenvironment{example}{\begin{interlude}\pagebreak[2]\noindent\textbf{Example.\ }\nopagebreak}{\enexample\end{interlude}}
%\newenvironment{examples}{\begin{interlude}\pagebreak[2]\noindent\textbf{Examples.\ }\nopagebreak}{\end{interlude}}
\newenvironment{smallexample}{\begin{smallinterlude}\pagebreak[2]\noindent\textbf{Example.\ }\nopagebreak}{\end{smallinterlude}}
%\newenvironment{examples}{\begin{interlude}\pagebreak[2]\noindent\textbf{Examples.\ }\nopagebreak\begin{enumsrm}\nopagebreak}{\end{enumsrm}\end{interlude}}
\newenvironment{examples*}{\begin{interlude}\pagebreak[2]\noindent\textbf{Beispiele.\ }\nopagebreak}{\end{interlude}}
%\newenvironment{notation}{\begin{interlude}\pagebreak[2]\noindent\textbf{Notation.\ }\nopagebreak}{\end{interlude}}
\newenvironment{notations}{\begin{interlude}\pagebreak[2]\noindent\textbf{Notationen.\ }\nopagebreak}{\end{interlude}}
\newenvironment{construction}{\begin{interlude}\pagebreak[2]\noindent\textbf{Construction.\ }\nopagebreak}{\end{interlude}}


\newenvironment{altproof}{\begin{interlude}\noindent\textit{alternativer Beweis.}}{\qed\end{interlude}}
\newenvironment{beweis}{\begin{interlude}\noindent\textit{Beweis.}}{\qed\end{interlude}}
\newenvironment{proof}{\begin{interlude}\noindent\textit{Proof.}}{\qed\end{interlude}}
\newenvironment{proofof}[1]{\begin{interlude}\noindent\textit{Beweis von} #1.}{\qed\end{interlude}}
\newenvironment{proof*}{\begin{interlude}\noindent\noindent\textit{Beweis.}}{\end{interlude}}


\newcommand\qedsymbol{$\square$}
\newcommand\enexamplesymbol{$\blacksquare$}
\newcommand\remarksymbol{$\underline{\quad\quad}$}
\newcommand\qed{\nopagebreak\penalty10000\hbox{}\nobreak\penalty10000\nopagebreak\penalty10000\hfill\hbox{\qedsymbol}\par}
\newcommand\enexample{\nopagebreak\penalty10000\hbox{}\nobreak\penalty10000\nopagebreak\penalty10000\hfill\hbox{\enexamplesymbol}\par}
\newcommand\remarkend{\nopagebreak\penalty10000\hbox{}\nobreak\penalty10000\nopagebreak\penalty10000\hfill\hbox{\remarksymbol}\par}


\newcommand{\zB}{\mbox{z.\,B}.\ }
\newcommand{\bzw}{\mbox{bzw}.\ }
\renewcommand{\dh}{\mbox{d.\,h}.\ }
\newcommand{\ua}{\mbox{u.\,a}.\ }
\newcommand{\ia}{\mbox{i.\,a}.\ }
\newcommand{\Dh}{\mbox{D.\,h}.\ }
\newcommand{\Cech}{\v{C}ech}


\newcommand\rmt[1]{{\rm #1}}




\def\TS{\textstyle}
\def\DS{\displaystyle}
\def\SSS{\scriptscriptstyle}
\def\SS{\scriptstyle}



\def\phi{\varphi}
\def\theta{\vartheta}
\def\epsilon{\varepsilon}
\def\sh{^\#}
\def\sub{\subseteq}
%\def\sup{\supseteq}
\def\subneq{\varsubsetneq}
\def\supneq{\varsupsetneq}
\def\nsub{\nsubseteq}
\def\nsup{\nsupseteq}

%\def\emptyset{\varnothing}


\newcommand\suml{\DS\sum\limits}
\newcommand\prodl{\DS\prod\limits}
\newcommand\coprodl{\DS\coprod\limits}
\newcommand\bigoplusl{\DS\bigoplus\limits}

%\def\mathbb{\mathds}

\newcommand\bbN{{\mathbb{N}}}
\newcommand\bbZ{{\mathbb{Z}}}
\newcommand\bbQ{{\mathbb{Q}}}
\newcommand\bbR{{\mathbb{R}}}
\newcommand\bbC{{\mathbb{C}}}
\newcommand\bbV{{\mathbb{V}}}
\newcommand\bbF{{\mathbb{F}}}
\newcommand\bbA{{\mathbb{A}}}
\newcommand\bbP{{\mathbb{P}}}
\newcommand\bbk{{\mathbb{k}}}
\newcommand\bbG{{\mathbb{G}}}



\newcommand\frakA{{\mathfrak{A}}}
\newcommand\frakN{{\mathfrak{N}}}
\newcommand\frakM{{\mathfrak{M}}}





\newcommand\powerset [1]{\mathfrak P\left(#1\right)}

\DeclareMathOperator{\id}{id} %
\DeclareMathOperator{\im}{im} %
\DeclareMathOperator{\coim}{coim} %
\DeclareMathOperator{\coker}{coker} %
\DeclareMathOperator{\preim}{pre\kern0.13em im} %
\DeclareMathOperator{\preker}{pre\kern0.13em ker} %
\DeclareMathOperator{\precoker}{pre\kern0.13em coker} %
\DeclareMathOperator{\pre}{pre} %
\DeclareMathOperator{\aut}{Aut} %
\DeclareMathOperator{\Endo}{End} %
\renewcommand{\hom}{\operatorname{Hom}}
\DeclareMathOperator{\bil}{Bil} %
\DeclareMathOperator{\dom}{dom} %
\DeclareMathOperator{\codom}{codom} %
\DeclareMathOperator{\mor}{Mor} %
\DeclareMathOperator{\der}{Der} %
\DeclareMathOperator{\tot}{Tot} %
\DeclareMathOperator{\grad}{grad} %
\DeclareMathOperator{\rg}{rg} %
\DeclareMathOperator{\sgn}{sgn} %
\DeclareMathOperator{\quot}{quot} %
\DeclareMathOperator{\ord}{ord} %
\DeclareMathOperator{\spec}{spec} %
\DeclareMathOperator{\spm}{spm} %
\DeclareMathOperator{\proj}{proj} %
\DeclareMathOperator{\rad}{rad} %
\DeclareMathOperator{\ass}{ass} %
\DeclareMathOperator{\supr}{sup} %
\DeclareMathOperator{\codim}{codim} %
\DeclareMathOperator{\hgt}{ht} %


\DeclareMathOperator{\supp}{supp} %

\DeclareMathOperator{\func}{Func} %

\DeclareMathOperator{\card}{card} %
\DeclareMathOperator{\pic}{Pic} %



\DeclareMathOperator{\ggT}{ggT} %
\DeclareMathOperator{\kgV}{kgV} %



\def\nin{\notin}
\def\nni{\not\ni}
\def\iso{\cong}

\def\homotop{\simeq}

\newcommand\fraka{\mathfrak a}
\newcommand\frakb{\mathfrak b}
\newcommand\frakc{\mathfrak c}
\newcommand\frakp{\mathfrak p}
\newcommand\frakq{\mathfrak q}
\newcommand\frakm{\mathfrak m}
\newcommand\frakn{\mathfrak n}

\newcommand\frakj{\mathfrak j}


\newcommand\defeq{\mathrel{\mathop:}=}
\newcommand\fedeq{=:}
\newcommand\then{\Rightarrow}
\newcommand\Then{\;\Longrightarrow\;}
\newcommand\neht{\Leftarrow}
\newcommand\Neht{\;\Longleftarrow\;}

\renewcommand\iff{\Leftrightarrow}
\newcommand\defiff{:\Leftrightarrow}
\newcommand\Iff{\;\Longleftrightarrow\;}
\newcommand\defIff{\;:\Longleftrightarrow\;}

\newcommand\set[2][auto]{
     \ifthenelse{\equal{#1}{auto}}{\left\lbrace}{\csname #1\endcsname\lbrace} #2 \ifthenelse{\equal{#1}{auto}}{\right\rbrace}{\csname #1\endcsname\rbrace} }



\newcommand\abs [1]{\left\vert #1 \right\vert}
\newcommand\norm [1]{\left\Vert #1 \right\Vert}
\newcommand\quotient [2]{{^{\DS #1 \!}\big\mod _{\DS#2}}}
\renewcommand\mod{/}
\newcommand\premod{\sslash}

\let\tensor\varotimes
\let\oplus\varoplus

\newcommand\bigtensor[1][]{\operatorname*{\sideset{}{_{#1}}\bigotimes}}


% Definitionen für Kategorientheorie --------------------------------------------------


\DeclareMathOperator\ob{Obj}

\newcommand{\indlim}{\operatorname*{\underrightarrow{\rm lim}}} %
\renewcommand{\projlim}{\operatorname*{\underleftarrow{\rm lim}}}


\DeclareMathOperator*\Indlim{\underrightarrow{\scrL\!\textit{im}}} %
\DeclareMathOperator*\Projlim{\underleftarrow{\scrL\!\textit{im}}} %
%\DeclareMathOperator\Indlim{\underrightarrow{\mathfrak{Lim}}} %
%\DeclareMathOperator\Projlim{\underleftarrow{\mathfrak{Lim}}} %



\newcommand\longto{\longrightarrow}
%\newcommand\isoto{\longto\!\!\!\!\!\!\!\!^\sim\,\,\,}
\newcommand\isoto{\mbox{$\hspace{7.5pt}\raise 3pt\hbox{$\sim$}\hspace{-17pt}\longrightarrow\hspace{3pt}$}\linebreak[0]}
\newcommand\isoot{\mbox{$\hspace{8.5pt}\raise 3pt\hbox{$\sim$}\hspace{-18pt}\longleftarrow\hspace{3pt}$}\linebreak[0]}
%\renewcommand\isoto{\stackrel{{}_\sim}\longto}
\newcommand\into{\hookrightarrow}
\newcommand\longinto{\lhook \joinrel \longrightarrow}
%\newcommand\onto{\twoheadrightarrow}
\newcommand\onto{\to\nolinebreak\hspace{-9.5pt}\to}
\newcommand\longonto{\longto\hspace{-9.5pt}\to}

\newcommand\To[1]{\stackrel {#1}\to}
\newcommand\Longto[1]{\stackrel {#1}\longto}
\newcommand\Longot[1]{\stackrel {#1}\longleftarrow}
\newcommand\Longinto[1]{\stackrel {#1}\longinto}
\newcommand\Longonto[1]{\stackrel {#1}\longonto}
\renewcommand\Longmapsto[1]{\stackrel {#1}\longmapsto}


%Einige Kategorien
\newcommand\Ab{{\mathfrak{Ab}}}


\newcommand\SET{{\mathbb{S}{\rm et}} }
\newcommand\MOD{{\mathbb{M}{\rm od}} }
\newcommand\RMOD[1][R]{{}_{#1}\MOD}
\newcommand\OxMOD{\RMOD[\scrO_X]}
\newcommand\AMOD{\RMOD[A]}
\newcommand\MODR[1][1]{\MOD_{#1}}
\newcommand\RMODS{{}_R\MOD_S}

\newcommand\AB{{\mathbb{A}{\rm b}}}
\newcommand\GRP{{\mathbb{G}{\rm rp}}}
\newcommand\TOP{{\mathbb{T}{\rm op}}}
\newcommand\RING{{\mathbb{R}{\rm ing}}}
\newcommand\FIELD{{\mathbb{F}{\rm ield}}}
\newcommand\ALG{{\mathbb{A}{\rm lg}} }
\newcommand\RALG[1][R]{{}_{#1}\ALG}
\newcommand\CAT{{\mathbb{C}{\rm at}}}
\newcommand\VAR{\mathbb{V}{\rm ar}}

\newcommand\qcMOD[1]{\!{\begin{smallmatrix}\hfill\rm qc\\ \hfill #1 \end{smallmatrix}\!\MOD}}


\newcommand\calA{\mathcal A}
\newcommand\calB{\mathcal B}
\newcommand\calC{\mathcal C}
\newcommand\calD{\mathcal D}
\newcommand\calE{\mathcal E}
\newcommand\calI{\mathcal I}
\newcommand\calP{\mathcal P}
\newcommand\calS{\mathcal S}
\newcommand\calX{\mathcal X}

\newcommand\op{^o}

\newcommand\ABAx[1]{\rmt{\bf(AB$#1$)}}
\newcommand\PSAx[1]{\rmt{\bf(PS$#1$)}}
\newcommand\TRAx[1]{\rmt{\bf(TR$#1$)}}
\newcommand\LCAx[1]{\rmt{\bf(LC$#1$)}}


% Homologische Algebra ----------------------------------------

\newcommand\ext{\operatorname{Ext}}
\newcommand\tor{\operatorname{Tor}}

\newcommand\ldot{_{\mathbf\cdot}}
\newcommand\udot{^{\mathbf\cdot}}

\newcommand{\HH}{{\rm H}} %
\newcommand{\BB}{{\rm B}} %
\newcommand{\ZZ}{{\rm Z}} %
\newcommand{\RR}{{\rm R}} %
\newcommand{\LL}{{\rm L}} %
\newcommand{\FF}{{\rm F}} %

\DeclareMathOperator{\gr}{gr} %

\newcommand{\cHH}{\check{\rm H}} %

\newcommand\ppH{{}''\HH} %
\newcommand\pH{{}'\HH} %
\newcommand\ppB{{}''\BB} %
\newcommand\pB{{}'\BB} %
\newcommand\ppZ{{}''\ZZ} %
\newcommand\pZ{{}'\ZZ} %
\newcommand\ppF{{}''\FF} %
\newcommand\pF{{}'\FF} %

\newcommand\ppE{{}''\!E} %
\newcommand\pE{{}'\!E} %


\newcommand\ssto{\Longrightarrow} %für _S_pektral_s_equenzen


\newcommand\del{\partial}

\newcommand\inm{\in_{\!\rm m}}
\newcommand\eqm{\equiv}

\DeclareMathOperator{\cone}{cone} %
\DeclareMathOperator{\tri}{Tri} %

\newcommand\triang[6]{
\begin{diagram}[width=0.3in,height=0.25in,tight]
  & #3 \\
\ldTo(1,2)<{#6}  & & \luTo(1,2)>{#5} \\
#1 & \rTo_{#4} & #2
\end{diagram}
}



\newcommand\roof[5]{
    \begin{diagram}[width=0.27in,height=0.23in,tight]
       &              & #2 \\
       & \ldTo(2,2)<{#4} &   & \rdTo(2,2)>{#5} \\
     #1 &              &   &              & #3
     \end{diagram}
}

\newcommand\roofd[5]{
    \begin{diagram}[width=0.27in,height=0.23in,tight]
       &              & #2 \\
       & \ruTo(2,2)<{#4} &   & \luTo(2,2)>{#5} \\
     #1 &              &   &              & #3
     \end{diagram}
}




\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}
